Saving Money for Analytical Workloads in the Cloud

As users migrate their analytical workloads to cloud databases, it is becoming just as important to reduce monetary costs as it is to optimize query runtime. In the cloud, a query is billed based on either its compute time or the amount of data it processes. We observe that analytical queries are either compute- or IO-bound and each query type executes cheaper in a different pricing model. We exploit this opportunity and propose methods to build cheaper execution plans across pricing models that complete within user-defined runtime constraints. We implement these methods and produce execution plans spanning multiple pricing models that reduce the monetary cost for workloads by as much as 56%. We reduce individual query costs by as much as 90%. The prices chosen by cloud vendors for cloud services also impact savings opportunities. To study this effect, we simulate our proposed methods with different cloud prices and observe that multi-cloud savings are robust to changes in cloud vendor prices. These results indicate the massive opportunity to save money by executing workloads across multiple pricing models.

==> sections/old_profiling_tbl/profiling_table.tex <==
\begin{table*}[htbp]
\centering
% \begin{tabularx}{\linewidth}{|c|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|}
\hline
Dataset & \multicolumn{3}{c|}{0} & \multicolumn{3}{c|}{1} & \multicolumn{3}{c|}{2} & \multicolumn{3}{c|}{3} & \multicolumn{3}{c|}{4} & \multicolumn{3}{c|}{5} & \multicolumn{3}{c|}{6} & \multicolumn{3}{c|}{7} & \multicolumn{3}{c|}{8} & \multicolumn{3}{c|}{9} & \multicolumn{3}{c|}{10} & \multicolumn{3}{c|}{11} & \multicolumn{3}{c|}{12} & \multicolumn{3}{c|}{13} & \multicolumn{3}{c|}{14} & \multicolumn{3}{c|}{15} & \multicolumn{3}{c|}{16} & \multicolumn{3}{c|}{17} & \multicolumn{3}{c|}{18} & \multicolumn{3}{c|}{19} & \multicolumn{3}{c|}{20} & \multicolumn{3}{c|}{21} & \multicolumn{3}{c|}{22} & \multicolumn{3}{c|}{23} \\ \hline\hline
0.15 & \multicolumn{1}{c|}{28.62} & \multicolumn{1}{c|}{1} & 0 & \multicolumn{1}{c|}{27.84} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{24.71} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{16.52} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{25.43} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{25.85} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{26.85} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{15.64} & \multicolumn{1}{c|}{N/A} & 0 & \multicolumn{1}{c|}{27.13} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{28.41} & \multicolumn{1}{c|}{1} & 0 & \multicolumn{1}{c|}{28.45} & \multicolumn{1}{c|}{1} & 0 & \multicolumn{1}{c|}{19.59} & \multicolumn{1}{c|}{N/A} & 0 & \multicolumn{1}{c|}{27.32} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{28.33} & \multicolumn{1}{c|}{1} & 0 & \multicolumn{1}{c|}{28.74} & \multicolumn{1}{c|}{1} & 0 & \multicolumn{1}{c|}{22.36} & \multicolumn{1}{c|}{N/A} & 0 & \multicolumn{1}{c|}{25.01} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{9.87} & \multicolumn{1}{c|}{145} & 0 & \multicolumn{1}{c|}{28.24} & \multicolumn{1}{c|}{1} & 0 & \multicolumn{1}{c|}{28.46} & \multicolumn{1}{c|}{1} & 0 & \multicolumn{1}{c|}{28.43} & \multicolumn{1}{c|}{1} & 0 & \multicolumn{1}{c|}{26.46} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{19.54} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{27.74} & \multicolumn{1}{c|}{2} & 0 \\ \hline
0.25 & \multicolumn{1}{c|}{44.47} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{43.13} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{39.7} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{24.78} & \multicolumn{1}{c|}{4} & 0 & \multicolumn{1}{c|}{39.11} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{39.89} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{41.52} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{22.56} & \multicolumn{1}{c|}{N/A} & 0 & \multicolumn{1}{c|}{41.89} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{44.08} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{44.12} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{29.2} & \multicolumn{1}{c|}{N/A} & 0 & \multicolumn{1}{c|}{42.27} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{43.96} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{44.58} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{33.9} & \multicolumn{1}{c|}{N/A} & 0 & \multicolumn{1}{c|}{38.42} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{13.68} & \multicolumn{1}{c|}{200} & 0 & \multicolumn{1}{c|}{43.69} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{44.1} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{44.13} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{40.88} & \multicolumn{1}{c|}{2} & 0 & \multicolumn{1}{c|}{29.66} & \multicolumn{1}{c|}{4} & 0 & \multicolumn{1}{c|}{42.98} & \multicolumn{1}{c|}{2} & 0 \\ \hline
0.5 & \multicolumn{1}{c|}{84.64} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{81.97} & \multicolumn{1}{c|}{4} & 0 & \multicolumn{1}{c|}{75.04} & \multicolumn{1}{c|}{4} & 0 & \multicolumn{1}{c|}{46.17} & \multicolumn{1}{c|}{6} & 0 & \multicolumn{1}{c|}{73.55} & \multicolumn{1}{c|}{5} & 0 & \multicolumn{1}{c|}{75.29} & \multicolumn{1}{c|}{5} & 0 & \multicolumn{1}{c|}{78.58} & \multicolumn{1}{c|}{4} & 0 & \multicolumn{1}{c|}{39.96} & \multicolumn{1}{c|}{N/A} & 0 & \multicolumn{1}{c|}{79.45} & \multicolumn{1}{c|}{4} & 0 & \multicolumn{1}{c|}{83.85} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{84.01} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{53.63} & \multicolumn{1}{c|}{N/A} & 0 & \multicolumn{1}{c|}{80.21} & \multicolumn{1}{c|}{4} & 0 & \multicolumn{1}{c|}{83.58} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{84.86} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{63.25} & \multicolumn{1}{c|}{N/A} & 0 & \multicolumn{1}{c|}{72.42} & \multicolumn{1}{c|}{5} & 0 & \multicolumn{1}{c|}{24.76} & \multicolumn{1}{c|}{362} & 0 & \multicolumn{1}{c|}{83.06} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{83.92} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{83.94} & \multicolumn{1}{c|}{3} & 0 & \multicolumn{1}{c|}{77.32} & \multicolumn{1}{c|}{4} & 0 & \multicolumn{1}{c|}{55.24} & \multicolumn{1}{c|}{7} & 0 & \multicolumn{1}{c|}{81.61} & \multicolumn{1}{c|}{4} & 0 \\ \hline
1.0 & \multicolumn{1}{c|}{158.39} & \multicolumn{1}{c|}{5} & 0 & \multicolumn{1}{c|}{153.32} & \multicolumn{1}{c|}{6} & 0 & \multicolumn{1}{c|}{139.03} & \multicolumn{1}{c|}{8} & 0 & \multicolumn{1}{c|}{83.94} & \multicolumn{1}{c|}{11} & 0 & \multicolumn{1}{c|}{135.59} & \multicolumn{1}{c|}{9} & 0 & \multicolumn{1}{c|}{140.2} & \multicolumn{1}{c|}{9} & 0 & \multicolumn{1}{c|}{146.48} & \multicolumn{1}{c|}{7} & 0 & \multicolumn{1}{c|}{67.6} & \multicolumn{1}{c|}{N/A} & 0 & \multicolumn{1}{c|}{148.16} & \multicolumn{1}{c|}{7} & 0 & \multicolumn{1}{c|}{157.01} & \multicolumn{1}{c|}{6} & 0 & \multicolumn{1}{c|}{156.87} & \multicolumn{1}{c|}{5} & 0 & \multicolumn{1}{c|}{95.3} & \multicolumn{1}{c|}{N/A} & 0 & \multicolumn{1}{c|}{149.56} & \multicolumn{1}{c|}{7} & 0 & \multicolumn{1}{c|}{156.33} & \multicolumn{1}{c|}{6} & 0 & \multicolumn{1}{c|}{158.98} & \multicolumn{1}{c|}{5} & 0 & \multicolumn{1}{c|}{116.61} & \multicolumn{1}{c|}{N/A} & 0 & \multicolumn{1}{c|}{134.75} & \multicolumn{1}{c|}{8} & 0 & \multicolumn{1}{c|}{43.5} & \multicolumn{1}{c|}{635} & 0 & \multicolumn{1}{c|}{155.71} & \multicolumn{1}{c|}{6} & 0 & \multicolumn{1}{c|}{156.62} & \multicolumn{1}{c|}{5} & 0 & \multicolumn{1}{c|}{157.22} & \multicolumn{1}{c|}{6} & 0 & \multicolumn{1}{c|}{143.85} & \multicolumn{1}{c|}{7} & 0 & \multicolumn{1}{c|}{99.73} & \multicolumn{1}{c|}{13} & 0 & \multicolumn{1}{c|}{152.39} & \multicolumn{1}{c|}{6} & 0 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}




==> sections/old_profiling_tbl/profiling_table2.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|ccc|ccc|ccc|ccc|}
\hline
Sample \%  & \multicolumn{3}{c|}{15}         & \multicolumn{3}{c|}{25}         & \multicolumn{3}{c|}{50}          & \multicolumn{3}{c|}{100}          \\ \hline
Dataset & \multicolumn{1}{c|}{Cost} & \multicolumn{1}{c|}{Iter} & \multicolumn{1}{c|}{Error} & \multicolumn{1}{c|}{Cost} & \multicolumn{1}{c|}{Iter} & \multicolumn{1}{c|}{Error} & \multicolumn{1}{c|}{Cost} & \multicolumn{1}{c|}{Iter} & \multicolumn{1}{c|}{Error} & \multicolumn{1}{c|}{Cost} & \multicolumn{1}{c|}{Iter} & \multicolumn{1}{c|}{Error} \\ \hline
0 & \multicolumn{1}{c|}{28.62} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{44.47} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{84.64} & \multicolumn{1}{c|}{3} & 0.03 & \multicolumn{1}{c|}{158.39} & \multicolumn{1}{c|}{5} & 0.0 \\ \hline
1 & \multicolumn{1}{c|}{27.84} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{43.13} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{81.97} & \multicolumn{1}{c|}{4} & 0.03 & \multicolumn{1}{c|}{153.32} & \multicolumn{1}{c|}{6} & 0.0 \\ \hline
2 & \multicolumn{1}{c|}{24.71} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{39.7} & \multicolumn{1}{c|}{3} & 0.04 & \multicolumn{1}{c|}{75.04} & \multicolumn{1}{c|}{4} & 0.04 & \multicolumn{1}{c|}{139.03} & \multicolumn{1}{c|}{8} & 0.0 \\ \hline
3 & \multicolumn{1}{c|}{16.52} & \multicolumn{1}{c|}{3} & 0.05 & \multicolumn{1}{c|}{24.78} & \multicolumn{1}{c|}{4} & 0.05 & \multicolumn{1}{c|}{46.17} & \multicolumn{1}{c|}{6} & 0.05 & \multicolumn{1}{c|}{83.94} & \multicolumn{1}{c|}{11} & 0.0 \\ \hline
4 & \multicolumn{1}{c|}{25.43} & \multicolumn{1}{c|}{2} & 0.04 & \multicolumn{1}{c|}{39.11} & \multicolumn{1}{c|}{3} & 0.04 & \multicolumn{1}{c|}{73.55} & \multicolumn{1}{c|}{5} & 0.04 & \multicolumn{1}{c|}{135.59} & \multicolumn{1}{c|}{9} & 0.0 \\ \hline
5 & \multicolumn{1}{c|}{25.85} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{39.89} & \multicolumn{1}{c|}{3} & 0.03 & \multicolumn{1}{c|}{75.29} & \multicolumn{1}{c|}{5} & 0.04 & \multicolumn{1}{c|}{140.2} & \multicolumn{1}{c|}{9} & 0.0 \\ \hline
6 & \multicolumn{1}{c|}{26.85} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{41.52} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{78.58} & \multicolumn{1}{c|}{4} & 0.04 & \multicolumn{1}{c|}{146.48} & \multicolumn{1}{c|}{7} & 0.0 \\ \hline
7 & \multicolumn{1}{c|}{15.64} & \multicolumn{1}{c|}{N/A} & 0.08 & \multicolumn{1}{c|}{22.56} & \multicolumn{1}{c|}{N/A} & 0.08 & \multicolumn{1}{c|}{39.96} & \multicolumn{1}{c|}{N/A} & 0.09 & \multicolumn{1}{c|}{67.6} & \multicolumn{1}{c|}{N/A} & 0.0 \\ \hline
8 & \multicolumn{1}{c|}{27.13} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{41.89} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{79.45} & \multicolumn{1}{c|}{4} & 0.04 & \multicolumn{1}{c|}{148.16} & \multicolumn{1}{c|}{7} & 0.0 \\ \hline
9 & \multicolumn{1}{c|}{28.41} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{44.08} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{83.85} & \multicolumn{1}{c|}{3} & 0.03 & \multicolumn{1}{c|}{157.01} & \multicolumn{1}{c|}{6} & 0.0 \\ \hline
10 & \multicolumn{1}{c|}{28.45} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{44.12} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{84.01} & \multicolumn{1}{c|}{3} & 0.04 & \multicolumn{1}{c|}{156.87} & \multicolumn{1}{c|}{5} & 0.0 \\ \hline
11 & \multicolumn{1}{c|}{19.59} & \multicolumn{1}{c|}{N/A} & 0.06 & \multicolumn{1}{c|}{29.2} & \multicolumn{1}{c|}{N/A} & 0.06 & \multicolumn{1}{c|}{53.63} & \multicolumn{1}{c|}{N/A} & 0.06 & \multicolumn{1}{c|}{95.3} & \multicolumn{1}{c|}{N/A} & 0.0 \\ \hline
12 & \multicolumn{1}{c|}{27.32} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{42.27} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{80.21} & \multicolumn{1}{c|}{4} & 0.04 & \multicolumn{1}{c|}{149.56} & \multicolumn{1}{c|}{7} & 0.0 \\ \hline
13 & \multicolumn{1}{c|}{28.33} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{43.96} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{83.58} & \multicolumn{1}{c|}{3} & 0.03 & \multicolumn{1}{c|}{156.33} & \multicolumn{1}{c|}{6} & 0.0 \\ \hline
14 & \multicolumn{1}{c|}{28.74} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{44.58} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{84.86} & \multicolumn{1}{c|}{3} & 0.03 & \multicolumn{1}{c|}{158.98} & \multicolumn{1}{c|}{5} & 0.0 \\ \hline
15 & \multicolumn{1}{c|}{22.36} & \multicolumn{1}{c|}{N/A} & 0.04 & \multicolumn{1}{c|}{33.9} & \multicolumn{1}{c|}{N/A} & 0.04 & \multicolumn{1}{c|}{63.25} & \multicolumn{1}{c|}{N/A} & 0.04 & \multicolumn{1}{c|}{116.61} & \multicolumn{1}{c|}{N/A} & 0.0 \\ \hline
16 & \multicolumn{1}{c|}{25.01} & \multicolumn{1}{c|}{2} & 0.04 & \multicolumn{1}{c|}{38.42} & \multicolumn{1}{c|}{3} & 0.04 & \multicolumn{1}{c|}{72.42} & \multicolumn{1}{c|}{5} & 0.04 & \multicolumn{1}{c|}{134.75} & \multicolumn{1}{c|}{8} & 0.0 \\ \hline
17 & \multicolumn{1}{c|}{9.87} & \multicolumn{1}{c|}{145} & 0.08 & \multicolumn{1}{c|}{13.68} & \multicolumn{1}{c|}{200} & 0.06 & \multicolumn{1}{c|}{24.76} & \multicolumn{1}{c|}{362} & 0.07 & \multicolumn{1}{c|}{43.5} & \multicolumn{1}{c|}{635} & 0.0 \\ \hline
18 & \multicolumn{1}{c|}{28.24} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{43.69} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{83.06} & \multicolumn{1}{c|}{3} & 0.03 & \multicolumn{1}{c|}{155.71} & \multicolumn{1}{c|}{6} & 0.0 \\ \hline
19 & \multicolumn{1}{c|}{28.46} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{44.1} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{83.92} & \multicolumn{1}{c|}{3} & 0.04 & \multicolumn{1}{c|}{156.62} & \multicolumn{1}{c|}{5} & 0.0 \\ \hline
20 & \multicolumn{1}{c|}{28.43} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{44.13} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{83.94} & \multicolumn{1}{c|}{3} & 0.03 & \multicolumn{1}{c|}{157.22} & \multicolumn{1}{c|}{6} & 0.0 \\ \hline
21 & \multicolumn{1}{c|}{26.46} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{40.88} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{77.32} & \multicolumn{1}{c|}{4} & 0.04 & \multicolumn{1}{c|}{143.85} & \multicolumn{1}{c|}{7} & 0.0 \\ \hline
22 & \multicolumn{1}{c|}{19.54} & \multicolumn{1}{c|}{3} & 0.05 & \multicolumn{1}{c|}{29.66} & \multicolumn{1}{c|}{4} & 0.05 & \multicolumn{1}{c|}{55.24} & \multicolumn{1}{c|}{7} & 0.05 & \multicolumn{1}{c|}{99.73} & \multicolumn{1}{c|}{13} & 0.0 \\ \hline
23 & \multicolumn{1}{c|}{27.74} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{42.98} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{81.61} & \multicolumn{1}{c|}{4} & 0.04 & \multicolumn{1}{c|}{152.39} & \multicolumn{1}{c|}{6} & 0.0 \\ \hline
\end{tabular}}
\caption{Profiling costs, iterations needed to compensate for profiling costs,
and estimation error for 15, 25, 50, and 100\% samples (GA1 1TB).  }
\label{tbl:profiling_sample}
\end{table}
% 0       & \multicolumn{1}{c|}{28.62}    & 1 & \multicolumn{1}{c|}{44.47}    & 2     & \multicolumn{1}{c|}{84.64}    & 3     & \multicolumn{1}{c|}{158.39}    & 5 \\ \hline
% 1       & \multicolumn{1}{c|}{27.84}    & 2 & \multicolumn{1}{c|}{43.13}    & 2     & \multicolumn{1}{c|}{81.97}    & 4     & \multicolumn{1}{c|}{153.32}    & 6 \\ \hline
% 2       & \multicolumn{1}{c|}{24.71}    & 2 & \multicolumn{1}{c|}{39.7}    & 3     & \multicolumn{1}{c|}{75.04}    & 4     & \multicolumn{1}{c|}{139.03}    & 8 \\ \hline
% 3       & \multicolumn{1}{c|}{16.52}    & 3 & \multicolumn{1}{c|}{24.78}    & 4     & \multicolumn{1}{c|}{46.17}    & 6     & \multicolumn{1}{c|}{83.94}    & 11 \\ \hline
% 4       & \multicolumn{1}{c|}{25.43}    & 2 & \multicolumn{1}{c|}{39.11}    & 3     & \multicolumn{1}{c|}{73.55}    & 5     & \multicolumn{1}{c|}{135.59}    & 9 \\ \hline
% 5       & \multicolumn{1}{c|}{25.85}    & 2 & \multicolumn{1}{c|}{39.89}    & 3     & \multicolumn{1}{c|}{75.29}    & 5     & \multicolumn{1}{c|}{140.2}    & 9 \\ \hline
% 6       & \multicolumn{1}{c|}{26.85}    & 2 & \multicolumn{1}{c|}{41.52}    & 2     & \multicolumn{1}{c|}{78.58}    & 4     & \multicolumn{1}{c|}{146.48}    & 7 \\ \hline
% 7       & \multicolumn{1}{c|}{15.64}    & N/A & \multicolumn{1}{c|}{22.56}    & N/A     & \multicolumn{1}{c|}{39.96}    & N/A     & \multicolumn{1}{c|}{67.6}    & N/A \\ \hline
% 8       & \multicolumn{1}{c|}{27.13}    & 2 & \multicolumn{1}{c|}{41.89}    & 2     & \multicolumn{1}{c|}{79.45}    & 4     & \multicolumn{1}{c|}{148.16}    & 7 \\ \hline
% 9       & \multicolumn{1}{c|}{28.41}    & 1 & \multicolumn{1}{c|}{44.08}    & 2     & \multicolumn{1}{c|}{83.85}    & 3     & \multicolumn{1}{c|}{157.01}    & 6 \\ \hline
% 10       & \multicolumn{1}{c|}{28.45}    & 1 & \multicolumn{1}{c|}{44.12}    & 2     & \multicolumn{1}{c|}{84.01}    & 3     & \multicolumn{1}{c|}{156.87}    & 5 \\ \hline
% 11       & \multicolumn{1}{c|}{19.59}    & N/A & \multicolumn{1}{c|}{29.2}    & N/A     & \multicolumn{1}{c|}{53.63}    & N/A     & \multicolumn{1}{c|}{95.3}    & N/A \\ \hline
% 12       & \multicolumn{1}{c|}{27.32}    & 2 & \multicolumn{1}{c|}{42.27}    & 2     & \multicolumn{1}{c|}{80.21}    & 4     & \multicolumn{1}{c|}{149.56}    & 7 \\ \hline
% 13       & \multicolumn{1}{c|}{28.33}    & 1 & \multicolumn{1}{c|}{43.96}    & 2     & \multicolumn{1}{c|}{83.58}    & 3     & \multicolumn{1}{c|}{156.33}    & 6 \\ \hline
% 14       & \multicolumn{1}{c|}{28.74}    & 1 & \multicolumn{1}{c|}{44.58}    & 2     & \multicolumn{1}{c|}{84.86}    & 3     & \multicolumn{1}{c|}{158.98}    & 5 \\ \hline
% 15       & \multicolumn{1}{c|}{22.36}    & N/A & \multicolumn{1}{c|}{33.9}    & N/A     & \multicolumn{1}{c|}{63.25}    & N/A     & \multicolumn{1}{c|}{116.61}    & N/A \\ \hline
% 16       & \multicolumn{1}{c|}{25.01}    & 2 & \multicolumn{1}{c|}{38.42}    & 3     & \multicolumn{1}{c|}{72.42}    & 5     & \multicolumn{1}{c|}{134.75}    & 8 \\ \hline
% 17       & \multicolumn{1}{c|}{9.87}    & 145 & \multicolumn{1}{c|}{13.68}    & 200     & \multicolumn{1}{c|}{24.76}    & 362     & \multicolumn{1}{c|}{43.5}    & 635 \\ \hline
% 18       & \multicolumn{1}{c|}{28.24}    & 1 & \multicolumn{1}{c|}{43.69}    & 2     & \multicolumn{1}{c|}{83.06}    & 3     & \multicolumn{1}{c|}{155.71}    & 6 \\ \hline
% 19       & \multicolumn{1}{c|}{28.46}    & 1 & \multicolumn{1}{c|}{44.1}    & 2     & \multicolumn{1}{c|}{83.92}    & 3     & \multicolumn{1}{c|}{156.62}    & 5 \\ \hline
% 20       & \multicolumn{1}{c|}{28.43}    & 1 & \multicolumn{1}{c|}{44.13}    & 2     & \multicolumn{1}{c|}{83.94}    & 3     & \multicolumn{1}{c|}{157.22}    & 6 \\ \hline
% 21       & \multicolumn{1}{c|}{26.46}    & 2 & \multicolumn{1}{c|}{40.88}    & 2     & \multicolumn{1}{c|}{77.32}    & 4     & \multicolumn{1}{c|}{143.85}    & 7 \\ \hline
% 22       & \multicolumn{1}{c|}{19.54}    & 3 & \multicolumn{1}{c|}{29.66}    & 4     & \multicolumn{1}{c|}{55.24}    & 7     & \multicolumn{1}{c|}{99.73}    & 13 \\ \hline
% 23       & \multicolumn{1}{c|}{27.74}    & 2 & \multicolumn{1}{c|}{42.98}    & 2     & \multicolumn{1}{c|}{81.61}    & 4     & \multicolumn{1}{c|}{152.39}    & 6 \\ \hline



==> sections/opt_soln.tex <==
\subsubsection{Optimal Solution}
We use a similar approach as Heller et. al.~\cite{rpsp}. We construct a capacity
function $c: E\rightarrow \R$ and a bipartite graph $G$ as above; nodes on the
left are tables and on the right are queries.  We draw \emph{directed} edges
with infinite capacity from tables to queries corresponding to query dependencies.
We add a source node $a$ and draw edges from $a$ to every table $t_i$; $c((a,
t_i)) = \mu_{t_i}$. We create a sink node $b$ and draw edges from every query
$q_j$ to $b$; $c((q_j, b)) = \sigma_{q_j}$ 
The algorithm computes the min-cut $C=(A,B)$ and designates the
set of queries and tables in $B$ to migrate to $X_d$.
We define $c(C)$ to be the capacity of edges spanning a cut $C$. 

We note that every potential solution to the inter-query optimization problem is
defined uniquely by the set of queries $W$ that move to $X_d$. We make two
claims showing that the solution corresponding to the min-cut of this graph
achieves the largest savings. 
% as it will be most effective to only move tables in
% $N^{-1}(W)$ to $X_d$. If more tables are moved than those in $N^{-1}(W)$, we pay
% unnecessary migration costs. 
% will be of the form $(W, N^{-1}(W))$, where $W$ is a subset
% of queries and $N^{-1}(W)$ is the set of tables required by $W$ as moving more
% tables pays unnecessary migration costs. 

% If we move fewer tables, this
% is an invalid solution as $W$ then cannot migrate, and if we move more we are
% paying unnecessary migration costs.

\mypar{Claim 1} For every potential solution $W\subset Q$ there is a
cut $C_W = (A, B)$ of finite capacity and vice versa.
% produces a cut with
%     finite capacity of the graph,
%     and every finite cut directly induces a solution $<W< N^{-1}(W)>$> 

\mypar{Claim 2} A solution with queries $W$ saves $\sum_{q\in Q}{\sigma_q} -
c(C_W)$.


\mypar{Proof of Claim 1} A cut has infinite capacity only if a query and a table
it depends on are on opposite sides of the cut.  Given a solution $W \subset Q$, let $B =
W \cup N^{-1}(W) \cup \{b\}$ and $A$ be the remaining nodes. All edges spanning
the cut are outbound from $a$ or inbound from $b$, so $C_W = (A,B)$ will have
finite capacity.

Equivalently, for a given finite cut $C = (A, B)$, let $W = B \cap Q$, i.e. $W$
is all queries in $B$. Then $N^{-1}(W) = B \cap T$, since otherwise an infinite
capacity edge would span $A$ and $B$ as there would either be an edge from $A$
to $W$ or from $B$ to some query in $A$. If $\overline{W} = Q \setminus W$, we
can write $B = \{b\} \cup W \cup N^{-1}(W)$ and $A = \{a\} \cup \overline{W}
\cup Q\setminus N^{-1}(W)$. 

\mypar{Proof of Claim 2}
Using the form for a cut given in Claim 1, for a set of queries $W$
and a resulting cut $C_W = (A, B)$ we can rewrite the exprssion for $c(C_W)$ to
show that the solution maximizing savings equivalently produces a min-cut of the
graph.
% know that:
\begin{align*}
    c(C_W) = \sum_{q\in \overline{W}}{\sigma_q} + \sum\limits_{t\in
    N^{-1}(W)}{\mu_t} &=
    \sum\limits_{q\in Q}{\sigma_q} - \sum\limits_{q\in W}{\sigma_q} +
    \sum\limits_{t\in N^{-1}(W)}{\mu_t} \\
    \implies \sum\limits_{q\in W}{\sigma_q} - \sum\limits_{t\in T_W}{\mu_t} &=
    \sum\limits_{q\in Q}{\sigma_q} - c(C_W)
\end{align*}
%
% Hence the solution which maximizes savings equivalently produces a min-cut of the
% graph.
%
\mypar{Complexity of Optimal Algorithm} Using the Ford-Fulkerson algorithm
~\cite{edmonds_karp}, the complexity is $O(|V||E|^2)$. Dinitz's algorithm brings
this complexity down to $O(|V|^2|E|)$~\cite{Dinitz2006}.

% \begin{myitemize}
% \item Establish that every valid solution to our problem is some set of queries
%     $W$ and the set of tables that they depend on $N(W)$ since all other options
%     are either inefficient or invalid
% \item Establish that every min-cut $\iff$ valid solution to our problem
% \item Rewrite the optimization problem equation for a proposed solution in terms
%     of its corresponding cut capacity using the above claims 
% \item Directly claim that the solution produced from the min cut will be the
%     cheapest option. Show this is true using simple proof by contradiction. 
% \item Discuss running time: Floyd-Fulkerson is $O(|V||E|^2)$. Dinic's algorithm
%     is $O(|V|^2|E|)$. It is possible others are more efficient that I am unaware
%     of (\notets{our algo is $O(n(n+m))$ where $n$ is number of tables, $m$
%     number of queries. Our algorithm is indepdent of the number of edges, which
% we can say means that our algorithm is independent of the complexity of queries,
% precisely its independent of the number of tables they scan}\notera{sounds good -- we just need to do a reasonable effort to cite an efficient algorithm, then explain the diff compared to greedy})
% \end{myitemize}


==> sections/profiling_table.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|ccc|ccc|ccc|ccc|}
\hline
Sample \%  & \multicolumn{3}{c|}{15}         & \multicolumn{3}{c|}{25}         & \multicolumn{3}{c|}{50}          & \multicolumn{3}{c|}{100}          \\ \hline
Dataset & \multicolumn{1}{c|}{Cost} & \multicolumn{1}{c|}{Iter} & \multicolumn{1}{c|}{Error} & \multicolumn{1}{c|}{Cost} & \multicolumn{1}{c|}{Iter} & \multicolumn{1}{c|}{Error} & \multicolumn{1}{c|}{Cost} & \multicolumn{1}{c|}{Iter} & \multicolumn{1}{c|}{Error} & \multicolumn{1}{c|}{Cost} & \multicolumn{1}{c|}{Iter} & \multicolumn{1}{c|}{Error} \\ \hline
DS-Derived 0 & \multicolumn{1}{c|}{30.66} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{49.77} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{95.93} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{180.02} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
DS-Derived 1 & \multicolumn{1}{c|}{30.31} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{49.16} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{94.71} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{177.78} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
DS-Derived 2 & \multicolumn{1}{c|}{27.63} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{44.87} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{86.1} & \multicolumn{1}{c|}{2} & 0.04 & \multicolumn{1}{c|}{159.84} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
DS-Derived 3 & \multicolumn{1}{c|}{17.68} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{28.42} & \multicolumn{1}{c|}{1} & 0.04 & \multicolumn{1}{c|}{54.74} & \multicolumn{1}{c|}{2} & 0.05 & \multicolumn{1}{c|}{99.0} & \multicolumn{1}{c|}{4} & 0.0 \\ \hline
DS-Derived 4 & \multicolumn{1}{c|}{25.79} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{41.67} & \multicolumn{1}{c|}{2} & 0.04 & \multicolumn{1}{c|}{79.62} & \multicolumn{1}{c|}{2} & 0.05 & \multicolumn{1}{c|}{145.9} & \multicolumn{1}{c|}{4} & 0.0 \\ \hline
DS-Derived 5 & \multicolumn{1}{c|}{26.3} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{42.53} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{80.66} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{151.33} & \multicolumn{1}{c|}{4} & 0.0 \\ \hline
DS-Derived 6 & \multicolumn{1}{c|}{27.76} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{44.82} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{85.28} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{160.26} & \multicolumn{1}{c|}{4} & 0.0 \\ \hline
DS-Derived 7 & \multicolumn{1}{c|}{13.88} & \multicolumn{1}{c|}{N/A} & 0.06 & \multicolumn{1}{c|}{21.92} & \multicolumn{1}{c|}{N/A} & 0.08 & \multicolumn{1}{c|}{39.39} & \multicolumn{1}{c|}{N/A} & 0.1 & \multicolumn{1}{c|}{65.6} & \multicolumn{1}{c|}{N/A} & 0.0 \\ \hline
DS-Derived 8 & \multicolumn{1}{c|}{28.48} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{45.97} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{87.55} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{165.11} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
DS-Derived 9 & \multicolumn{1}{c|}{30.27} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{49.06} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{94.51} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{177.33} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
DS-Derived 10 & \multicolumn{1}{c|}{30.41} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{49.34} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{95.07} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{178.27} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
DS-Derived 11 & \multicolumn{1}{c|}{19.42} & \multicolumn{1}{c|}{5} & 0.04 & \multicolumn{1}{c|}{30.89} & \multicolumn{1}{c|}{8} & 0.05 & \multicolumn{1}{c|}{58.53} & \multicolumn{1}{c|}{15} & 0.06 & \multicolumn{1}{c|}{104.09} & \multicolumn{1}{c|}{26} & 0.0 \\ \hline
DS-Derived 12 & \multicolumn{1}{c|}{29.22} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{47.32} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{91.0} & \multicolumn{1}{c|}{2} & 0.04 & \multicolumn{1}{c|}{170.08} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
DS-Derived 13 & \multicolumn{1}{c|}{30.07} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{48.71} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{93.84} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{175.86} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
DS-Derived 14 & \multicolumn{1}{c|}{30.69} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{49.88} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{95.94} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{180.2} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
DS-Derived 15 & \multicolumn{1}{c|}{22.96} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{36.79} & \multicolumn{1}{c|}{2} & 0.04 & \multicolumn{1}{c|}{69.02} & \multicolumn{1}{c|}{4} & 0.04 & \multicolumn{1}{c|}{129.0} & \multicolumn{1}{c|}{6} & 0.0 \\ \hline
DS-Derived 16 & \multicolumn{1}{c|}{26.75} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{43.28} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{83.05} & \multicolumn{1}{c|}{2} & 0.04 & \multicolumn{1}{c|}{154.22} & \multicolumn{1}{c|}{4} & 0.0 \\ \hline
DS-Derived 17 & \multicolumn{1}{c|}{8.7} & \multicolumn{1}{c|}{26} & 0.05 & \multicolumn{1}{c|}{13.55} & \multicolumn{1}{c|}{40} & 0.06 & \multicolumn{1}{c|}{25.0} & \multicolumn{1}{c|}{73} & 0.07 & \multicolumn{1}{c|}{43.61} & \multicolumn{1}{c|}{127} & 0.0 \\ \hline
DS-Derived 18 & \multicolumn{1}{c|}{30.03} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{48.73} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{93.65} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{175.89} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
DS-Derived 19 & \multicolumn{1}{c|}{30.31} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{49.27} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{94.72} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{177.49} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
DS-Derived 20 & \multicolumn{1}{c|}{30.57} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{49.61} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{95.6} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{179.65} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
DS-Derived 21 & \multicolumn{1}{c|}{28.57} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{46.39} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{89.11} & \multicolumn{1}{c|}{2} & 0.04 & \multicolumn{1}{c|}{166.24} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
DS-Derived 22 & \multicolumn{1}{c|}{20.73} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{33.59} & \multicolumn{1}{c|}{2} & 0.04 & \multicolumn{1}{c|}{64.38} & \multicolumn{1}{c|}{3} & 0.06 & \multicolumn{1}{c|}{115.65} & \multicolumn{1}{c|}{5} & 0.0 \\ \hline
DS-Derived 23 & \multicolumn{1}{c|}{30.16} & \multicolumn{1}{c|}{1} & 0.02 & \multicolumn{1}{c|}{48.91} & \multicolumn{1}{c|}{1} & 0.03 & \multicolumn{1}{c|}{94.22} & \multicolumn{1}{c|}{2} & 0.03 & \multicolumn{1}{c|}{176.73} & \multicolumn{1}{c|}{3} & 0.0 \\ \hline
\end{tabular}}
\caption{Profiling costs, iterations needed to compensate for profiling costs,
and estimation error for 15, 25, 50, and 100\% samples (GA1 1TB).  }
\label{tbl:profiling_sample}
\end{table}



==> sections/sql_preopt_tables.tex <==
% \begin{table}[]
% \resizebox{0.6\columnwidth}{!}{
% \begin{tabular}{|c|c|c|}
% \hline
% Query        & \% Speedup & Difference \\ \hline
% 04           & 54.82      & Append Order          \\ \hline
% 09           & -56.08     & Join Order/Algorithm  \\ \hline
% 18           & 72.76      & Append Order          \\ \hline
% 22           & 29.57      & Append Order          \\ \hline
% 25           & 96.28      & Join Order            \\ \hline
% 27           & 14.23      & Append Order          \\ \hline
% 33           & -23.90     & Join Order            \\ \hline
% 48           & -52.90     & Join Order            \\ \hline
% 49           & -5.54      & Append Order          \\ \hline
% 56           & -204.96    & Append Order          \\ \hline
% 60           & 79.03      & Append Order          \\ \hline
% 71           & 9.80       & Join \& Append Order  \\ \hline
% 72           & 46.88      & Join Order, Filter    \\ \hline
% 75           & 10.72      & Append Order          \\ \hline
% 83           & -33.02     &                       \\ \hline
% 84           & 71.58      & Join Order            \\ \hline
% 87           & 47.43      & Append Order          \\ \hline
% 95           & -379.41    & Join Order            \\ \hline
% \end{tabular}}
% \caption{TPC-DS queries that produced different query plans in Redshift based on
% SQL syntax, along with the \% speedup of the machine-generated SQL and a short
% description of the difference in query plans}
% \label{tbl:rs_preop}
% \end{table}

% \begin{table}[]
% \resizebox{0.45\columnwidth}{!}{
% \begin{tabular}{|c|c|c|}
% \hline
% Query        & \% Speedup & Difference \\ \hline \hline
% 03           & -28.21     & Join Order             \\ \hline
% 04           & 3.02       & Join Order             \\ \hline
% 11           & 20.92      & Join Order             \\ \hline
% 15           & 9.61       & Join Order             \\ \hline
% 19           & 19.57      & Join Order             \\ \hline
% 21           & -22.22     & Join Order             \\ \hline
% 34           & -0.46      & Join Order             \\ \hline
% 37           & 97.72      & Join Order             \\ \hline
% 39           & -40.20     & Join Order             \\ \hline
% 40           & -23.27     & Join Order             \\ \hline
% 42           & 10.04      & Join Order             \\ \hline
% 43           & -45.21     & Join Order             \\ \hline
% 46           & -4.59      & Join Order             \\ \hline
% 47           & -272.41    & Join Order             \\ \hline
% 50           & -7.39      & Join Order             \\ \hline
% 52           & -24.28     & Join Order             \\ \hline
% 55           & 1.28       & Join Order             \\ \hline
% 56           & -11.35     & Join Order             \\ \hline
% 57           & -279.11    & Join Order             \\ \hline
% 60           & -18.08     & Join Order             \\ \hline
% 63           & 4.23       & Join Order             \\ \hline
% 68           & -7.36      & Join Order             \\ \hline
% 73           & 2.53       & Join Order             \\ \hline
% 74           & -72.13     & Join Order             \\ \hline
% 79           & 9.40       & Join Order             \\ \hline
% 82           & 97.49      & Join Order             \\ \hline
% 89           & -21.95     & Join Order             \\ \hline
% 91           & -65.33     & Join Order             \\ \hline
% \end{tabular}}
% \caption{TPC-DS queries that produced different query plans in DuckDB based on
% SQL syntax, along with the \% speedup of the machine-generated SQL and a short
% description of the difference in query plans}
% \label{tbl:duck_preop}
% \end{table}



==> sections/unused_tables.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
Dataset &  Profiling Cost (\$) & Iterations & Plan-Type \\ \hline \hline
0 &  158.3902903187325 &  5 & aws \\ \hline
1 &  153.31870822480755 &  6 & aws \\ \hline
2 &  139.03425230384414 &  8 & multi \\ \hline
3 &  83.9408997423685 &  11 & multi \\ \hline
4 &  135.58545926714692 &  9 & aws \\ \hline
5 &  140.20221297525518 &  9 & aws \\ \hline
6 &  146.47703111015676 &  7 & aws \\ \hline
7 &  67.59563129566068 &  N/A & gcp \\ \hline
8 &  148.1553903276047 &  7 & aws \\ \hline
9 &  157.01193859953202 &  6 & aws \\ \hline
10 &  156.8714283896223 &  5 & aws \\ \hline
11 &  95.30218658024006 &  N/A & gcp \\ \hline
12 &  149.56448712892765 &  7 & aws \\ \hline
13 &  156.32525955666375 &  6 & aws \\ \hline
14 &  158.97986169735833 &  5 & aws \\ \hline
15 &  116.60617279408618 &  1702 & multi \\ \hline
16 &  134.74555828414034 &  8 & multi \\ \hline
17 &  43.497958788464665 &  635 & multi \\ \hline
18 &  155.7066822981122 &  6 & aws \\ \hline
19 &  156.6242319566121 &  5 & multi \\ \hline
20 &  157.21691238205054 &  6 & aws \\ \hline
21 &  143.853411530078 &  7 & aws \\ \hline
22 &  99.72802733276917 &  13 & multi \\ \hline
23 &  152.39025357863838 &  6 & aws \\ \hline
\end{tabular}
\caption{GA1 1TB: Profiling costs, number of iterations for savings to makeup for
profiling costs, and plan type for each dataset}
\label{tbl:ga1_1_profiling}
\end{table}

\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
Dataset &  Profiling Cost (\$) & Iterations & Plan-Type \\ \hline \hline
0 &  163.4650350122072 &  6 & aws \\ \hline
1 &  158.11345750111957 &  7 & aws \\ \hline
2 &  142.92856660355397 &  9 & multi \\ \hline
3 &  86.7816291617738 &  13 & multi \\ \hline
4 &  138.7026227756748 &  11 & aws \\ \hline
5 &  143.72391345306673 &  11 & aws \\ \hline
6 &  150.40907633694212 &  8 & aws \\ \hline
7 &  68.18502295975235 &  N/A & gcp \\ \hline
8 &  152.97280618599538 &  8 & aws \\ \hline
9 &  161.9128374684087 &  6 & aws \\ \hline
10 &  161.89190967776335 &  6 & aws \\ \hline
11 &  98.63877239011791 &  N/A & gcp \\ \hline
12 &  154.1567416213153 &  8 & aws \\ \hline
13 &  161.38541122738707 &  6 & aws \\ \hline
14 &  164.00247869258948 &  6 & aws \\ \hline
15 &  120.11488056335732 &  4950 & multi \\ \hline
16 &  138.37331788864793 &  10 & multi \\ \hline
17 &  44.52608316481924 &  1835 & multi \\ \hline
18 &  160.6596656363672 &  7 & aws \\ \hline
19 &  161.63242414957705 &  6 & multi \\ \hline
20 &  162.0895349860151 &  6 & aws \\ \hline
21 &  147.84702023065532 &  9 & aws \\ \hline
22 &  102.24632901060642 &  16 & multi \\ \hline
23 &  157.24637332431791 &  7 & aws \\ \hline
\end{tabular}
\caption{GA4 1TB: Profiling costs, number of iterations for savings to makeup for
profiling costs, and plan type for each dataset}
\label{tbl:ga1_4_profiling}
\end{table}


\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
Dataset &  Profiling Cost (\$) & Iterations & Plan-Type \\ \hline \hline
0 &  352.42978508326144 &  3 & aws \\ \hline
1 &  337.5068872799689 &  3 & aws \\ \hline
2 &  302.6987030123627 &  4 & multi \\ \hline
3 &  178.29379424973524 &  5 & multi \\ \hline
4 &  294.43333110381116 &  4 & aws \\ \hline
5 &  306.2381572013433 &  4 & aws \\ \hline
6 &  320.73884420845764 &  4 & aws \\ \hline
7 &  123.99848969616777 &  N/A & gcp \\ \hline
8 &  328.0671422164779 &  4 & aws \\ \hline
9 &  348.17087398775766 &  3 & aws \\ \hline
10 &  354.10037686795056 &  3 & aws \\ \hline
11 &  198.0998829036264 &  310 & multi \\ \hline
12 &  330.0367677639593 &  4 & aws \\ \hline
13 &  346.2869119138671 &  3 & aws \\ \hline
14 &  353.3563320616101 &  3 & aws \\ \hline
15 &  243.46249642538362 &  7 & aws \\ \hline
16 &  290.4545191684344 &  4 & multi \\ \hline
17 &  77.18886956704635 &  N/A & gcp \\ \hline
18 &  345.8813309664971 &  3 & aws \\ \hline
19 &  351.36111466999404 &  3 & aws \\ \hline
20 &  347.7126961699943 &  3 & aws \\ \hline
21 &  312.9974329183479 &  4 & aws \\ \hline
22 &  210.52811014804496 &  6 & multi \\ \hline
23 &  335.7796444882932 &  3 & aws \\ \hline
\end{tabular}
\caption{GA1 2TB: Profiling costs, number of iterations for savings to makeup for
profiling costs, and plan type for each dataset}
\label{tbl:ga1_2_profiling}
\end{table}


\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
Dataset &  Profiling Cost (\$) & Iterations & Plan-Type \\ \hline \hline
0 &  351.582294803637 &  3 & aws \\ \hline
1 &  336.4075268257289 &  3 & aws \\ \hline
2 &  301.5949944690255 &  4 & multi \\ \hline
3 &  178.28339210177379 &  5 & multi \\ \hline
4 &  292.6881226339262 &  4 & aws \\ \hline
5 &  305.06957631997346 &  4 & aws \\ \hline
6 &  319.7653794053592 &  4 & aws \\ \hline
7 &  124.02782050372544 &  N/A & gcp \\ \hline
8 &  328.0724904513821 &  4 & aws \\ \hline
9 &  347.25803818897623 &  3 & aws \\ \hline
10 &  353.29851238578914 &  3 & aws \\ \hline
11 &  198.34602628017393 &  532 & multi \\ \hline
12 &  329.2214910477471 &  3 & aws \\ \hline
13 &  345.21111370541263 &  3 & aws \\ \hline
14 &  352.53506328840734 &  3 & aws \\ \hline
15 &  244.65591486530477 &  8 & aws \\ \hline
16 &  289.82173676192156 &  4 & multi \\ \hline
17 &  77.31782701368894 &  N/A & gcp \\ \hline
18 &  345.60239018508673 &  3 & aws \\ \hline
19 &  350.6002296841039 &  3 & aws \\ \hline
20 &  346.7304153182508 &  3 & aws \\ \hline
21 &  311.8303541561707 &  4 & aws \\ \hline
22 &  208.9049648681496 &  5 & multi \\ \hline
23 &  334.79607911254345 &  3 & aws \\ \hline
\end{tabular}
\caption{GA4 2TB: Profiling costs, number of iterations for savings to makeup for
profiling costs, and plan type for each dataset}
\label{tbl:ga4_2_profiling}
\end{table}


